Inferring Concise Specifications of APIs

Modern software relies on libraries and uses them via application programming interfaces (APIs). Correct API usage as well as many software engineering tasks are enabled when APIs have formal specifications. In this work, we analyze the implementation of each method in an API to infer a formal postcondition. Conventional wisdom is that, if one has preconditions, then one can use the strongest postcondition predicate transformer (SP) to infer postconditions. However, SP yields postconditions that are exponentially large, which makes them difficult to use, either by humans or by tools. Our key idea is an algorithm that converts such exponentially large specifications into a form that is more concise and thus more usable. This is done by leveraging the structure of the specifications that result from the use of SP. We applied our technique to infer postconditions for over 2,300 methods in seven popular Java libraries. Our technique was able to infer specifications for 75.7% of these methods, each of which was verified using an Extended Static Checker. We also found that 84.6% of resulting specifications were less than 1/4 page (20 lines) in length. Our technique was able to reduce the length of SMT proofs needed for verifying implementations by 76.7% and reduced prover execution time by 26.7%.

==> annonymous-authors.tex <==

\author{}


\Copyright{Annonymous Author(s)} %mandatory, please use full first names. LIPIcs license is "CC-BY";  http://creativecommons.org/licenses/by/3.0/


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> author-block.tex <==

\author[1]{John L. Singleton}
\affil[1]{University of Central Florida, Orlando, USA\\
  \texttt{jls@cs.ucf.edu}}

\author[2]{Gary T. Leavens}
\affil[2]{University of Central Florida, Orlando, USA\\
  \texttt{leavens@cs.ucf.edu}}


\author[3]{Hridesh Rajan}
\affil[3]{Iowa State University, Ames, USA\\
  \texttt{hridesh@iastate.edu}}


\author[4]{David R. Cok}
\affil[4]{GrammaTech, Inc, USA\\
  \texttt{dcok@grammatech.com}}


\Copyright{John L. Singleton, Gary T. Leavens, Hridesh Rajan, and David R. Cok} %mandatory, please use full first names. LIPIcs license is "CC-BY";  http://creativecommons.org/licenses/by/3.0/


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> calculation.tex <==
% $Id$
%
% Calculational proofs, a la Dijkstra, Gries, Back and von Wright, etc.
% See: David Gries, "Teaching Calculation and Discrimination:
%      A More Effective Curriculum", CACM 34(3):44-55, Mar. 1991.
% and
%      Ralph-Johan Back and Joakim von Wright,
%      "Refinement Calculus: A Systematic Introduction",
%      Springer-Verlag, 1998.
%
% AUTHOR: Gary T. Leavens

% EXAMPLES
%
% A simple example of the use of these macros is as follows.
%
% \begin{calculation}
% \FORMULA{\vec{RD}}
% \EQREASON{definition of $\vec{RD}$}
% \FORMULA{(RD_1, \ldots, RD_j, \ldots, RD_{12})}
% \REASON{\sqsubseteq}{$F_j$ is monotonic}
% \FORMULA{(RD_1, \ldots, F_j(\vec{RD}), \ldots, RD_{12})}
% \EQREASON{definition of $\vec{RD'}$}
% \LASTFORMULA{\vec{RD'}}
% \end{calculation}
%
% The following is a slightly more advanced example.
%
% \begin{calculation}
% \FORMULA{F(\vec{RD'}) \sqsubseteq \FOCUS{F^n(\vec{\emptyset})}}
% \EQREASON{assumption $F^n(\vec{\emptyset}) = F^{n+1}(\vec{\emptyset})$}
% \FORMULA{F(\vec{RD'}) \sqsubseteq \FOCUS{F^{n+1}(\vec{\emptyset})}}
% \EQREASON{definition of iteration of a function}
% \FORMULA{F(\vec{RD'}) \sqsubseteq F(F^n(\vec{\emptyset}))}
% \REASON{\impliedby}{monotonicity of $F$}
% \FORMULA{\vec{RD'} \sqsubseteq F^n(\vec{\emptyset})}
% \REASON{\impliedby}{transitivity}
% \FORMULA{\vec{RD'} \sqsubseteq F(\vec{RD})
%         \wedge F(\vec{RD}) \sqsubseteq F^n(\vec{\emptyset})}
% \EQREASON{assumption $F(\vec{RD}) \sqsubseteq F^n(\vec{\emptyset})$}
% \FORMULA{\vec{RD'} \sqsubseteq F(\vec{RD})}
% \REASON{\impliedby}{Lemma~7}
% \QEDFORMULA{\vec{RD} \sqsubseteq F(\vec{RD})}
% \end{calculation}
%
% An much more sophisticated example, with subdeductions a la Back and
% von Wright is the following.
%
% \begin{calculation}
% \FORMULA{\alpha(\{tr: (z, \ell') \mid tr \in \gamma(RD_k)\}) }
% \EQREASON{definition of $\alpha$}
% \FORMULA{\{(x, SRD(tr')(x))
%              \mid x \in \textrm{dom}(tr')
%                   \wedge tr' \in \{tr: (z, \ell') \mid tr \in \gamma(RD_k)\} \} }
% \EQREASON{set theory
%          ($tr'$ ranges over $tr: (z, \ell')$ for $tr \in \gamma(RD_k)$)}
% \FORMULA{\{(x, SRD(tr: (z, \ell'))(x))
%              \mid x \in \textrm{dom}(tr: (z, \ell')),
%                    \FOCUS{tr \in \gamma(RD_k)} \} }
% \EQREASON{definition of $\gamma$}
% \FORMULA{\{(x, SRD(tr: (z, \ell'))(x))
%              \mid x \in \textrm{dom}(tr: (z, \ell')),
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}}
% \EQREASON{set theory}
% \FORMULA{
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} \\
%         \cup \:
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x = z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%     \end{array}
%         }
% \EQREASON{focusing on the second set}
% \SUBDEDUCTION{
%      \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x = z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%      \end{array}
%        }
%   \EQREASON{set theory}
%   \FORMULA{\{(z, \FOCUS{SRD(tr: (z, \ell'))(z)}) 
%              \mid z \in \textrm{dom}(tr: (z, \ell')),
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} }
%   \EQREASON{definition of $SRD$}
%   \FORMULA{\{(z, \ell') 
%              \mid \FOCUS{z \in \textrm{dom}(tr: (z, \ell'))},
%                (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k)
%              \} }
%   \EQREASON{definition of $\textrm{dom}$}
%   \FORMULA{\{(z, \ell') 
%              \mid (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} }
%   \EQREASON{definition of $\gamma$}
%   \FORMULA{\{(z, \ell') \mid tr \in \gamma(RD_k) \} }
%   \EQREASON{$tr$ can be constructed by writing the pairs of
%              $\gamma(RD_k)$ in some order}
%   \FORMULA{\{(z, \ell') \} }
% \CONCLUDE{
%    \begin{array}{l}
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%     \end{array} \\
%     \cup \: \{(z, \ell')\}
%    \end{array}
%     }
% \EQREASON{focusing on the first set}
% \SUBDEDUCTION{
%     \begin{array}{rl}
%         \{(x, SRD(tr: (z, \ell'))(x)) &
%              \mid x \neq z, x \in \textrm{dom}(tr: (z, \ell')), \\
%              & ~ (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}
%      \end{array}
%        }
%   \EQREASON{definition of $SRD$}
%   \FORMULA{\{(x, SRD(tr)(x))
%              \mid x \neq z, x \in \textrm{dom}(tr), 
%               (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \}}
%   \EQREASON{set theory and the range of $SRD$}
%   \FORMULA{\begin{array}{l}
%              \{(x, SRD(tr)(x))
%                       \mid x \in \textrm{dom}(tr), 
%               (\forall y \in \textrm{dom}(tr) :: (y, SRD(tr)(y)) \in RD_k) \} \\
%            \setminus \: \{(z, \ell) \mid \ell \in \Lab\}
%            \end{array}
%           }
%   \EQREASON{Lemma \ref{lemma:simplifyToRD}}
%   \FORMULA{RD_k \setminus \{(z, \ell) \mid \ell \in \Lab\}}
% \LASTCONCLUDE{(RD_k \setminus \{(z, \ell) \mid \ell \in \Lab\})
%            \cup \{(z, \ell')\}}
% \end{calculation}


%%%%%%% The macros themselves follow %%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% You may want to define the following with \renewcommand...

% Brackets around normal and fixed width reasons
\newcommand{\LEFTREASONBRACKET}{\langle}
\newcommand{\RIGHTREASONBRACKET}{\rangle}
% Brackets for long reasons
\newcommand{\LONGLEFTREASONBRACKET}{\left\LEFTREASONBRACKET}
\newcommand{\LONGRIGHTREASONBRACKET}{\right\RIGHTREASONBRACKET}
% width of long and fixed width reasons
\newcommand{\LONGREASONWIDTH}{5.4in}
\newcommand{\FIXEDWIDTHREASONWIDTH}{\LONGREASONWIDTH}
% The phrase that starts each reason
\newcommand{\BYPHRASE}{by~}
% Provability symbol
\newcommand{\PROVABILITYSYMBOL}{\vdash}
% Has type symbol
\newcommand{\CALCULATIONHASTYPE}{:}
% Subdeduction symbols a la Back and von Wright
\newcommand{\SUBDEDUCTIONMARKER}{\bullet}
\newcommand{\CONCLUDEMARKER}{\cdot}

% The macros below assume that you have defined \QED,
% e.g., as \newcommand{\QED}{q.e.d.}


%%% The rest shouldn't usually need to be redefined

% The main environment
\newenvironment{calculation}{
\samepage
\begin{tabbing}
mm \= n \= mm \= n \= mm \= n \= mm \= n \= mm \= n \= mm \= n \= \kill
}{
\end{tabbing}
}

% Use for the last formula (to avoid extra vertical space)
\newcommand{\LASTFORMULA}[1]{\> \ensuremath{#1}}
% Use for the last formula in a proof that concluses the proof
\newcommand{\QEDATEND}{~~\QED}
\newcommand{\QEDFORMULA}[1]{\LASTFORMULA{#1\QEDATEND}}

% All other formulas in a calculation
\newcommand{\FORMULA}[1]{\LASTFORMULA{#1} \\}

% Generic reason, with connective and the justification
\newcommand{\REASON}[2]{%
    \ensuremath{#1}\> \>
       \mbox{\ensuremath{\LEFTREASONBRACKET}{\BYPHRASE}#2\ensuremath{\RIGHTREASONBRACKET}} \\}

% Reasons with longer justifications, with the right bracket at the end
\newcommand{\FIXEDWIDTHREASON}[2]{%
     \ensuremath{#1}\> \>
       \ensuremath{\LEFTREASONBRACKET}{\BYPHRASE}%
       \parbox[t]{\FIXEDWIDTHREASONWIDTH}{#2\ensuremath{\RIGHTREASONBRACKET}}
       \\
     }

% Reasons with longer justifications, with big brackets around the reason
\newcommand{\LONGREASON}[2]{%
    \ensuremath{#1}\> \>
      \ensuremath{\LONGLEFTREASONBRACKET
                  \parbox[c]{\LONGREASONWIDTH}{{\BYPHRASE}#2}
                  \LONGRIGHTREASONBRACKET
                 }
      \\
    }

% Specialization of reasons to equality
\newcommand{\EQREASON}[1]{\REASON{=}{#1}}
\newcommand{\EQLONGREASON}[1]{\LONGREASON{=}{#1}}
\newcommand{\EQFIXEDWIDTHREASON}[1]{\FIXEDWIDTHREASON{=}{#1}}

% Use \FOCUS{E} to say that subformula E will be changed in the following step
\newcommand{\FOCUS}[1]{\mbox{``}#1\mbox{''}}


%% The following are for Back and von Wright style calculations.
%% First time users may want to ignore these.

% Use for assumptions in a type-deduction style proof
\newcommand{\GIVEN}[1]{\FORMULA{#1}}
% Use \PROVETHAT to start the body of a type-deduction style proof.
\newcommand{\PROOFLINE}[2]{\ensuremath{#1} \> \ensuremath{#2} \\}
\newcommand{\PROVETHAT}[1]{\PROOFLINE{\PROVABILITYSYMBOL}{#1}}
%% Subdeductions
% Use to start a subdeduction
\newcommand{\SUBDEDUCTION}[1]{\+\+\kill\PROOFLINE{\SUBDEDUCTIONMARKER}{#1}}
% Use to separate one subdeduction from another
\newcommand{\ANDALSO}{\-\-\kill}
% Use to start the next subdeduction after \ANDALSO
\newcommand{\NEXTDEDUCTION}[1]{\PROOFLINE{\SUBDEDUCTIONMARKER}{#1}}
% Use to conclude a subdeduction 
\newcommand{\CONCLUDE}[1]{\-\-\kill\PROOFLINE{\CONCLUDEMARKER}{#1}}
% Use when the last formula is also a conclusion
\newcommand{\LASTCONCLUDE}[1]{\-\-\kill\ensuremath{\CONCLUDEMARKER} \> \ensuremath{#1}}
% Use in a type-deduction proof instead of \REASON, to give the rule name
\newcommand{\TYPINGRULE}[1]{\ensuremath{\CALCULATIONHASTYPE} \> ~~~ #1 \\}

% end of calculation.tex



==> correct.tex <==
\section{The \FAR Algorithm}
\label{sec:soundness}\label{sec:far-algorithm}


The main problem with formulas computed by \textit{sp} is that when the results are converted into specifications, they can become very large, deeply nested, and repetitive. At each branch point in the program the branch's precondition is fed back into \textit{sp} (see Equation \ref{eqn:if}) as an argument, which causes the number of specification cases in the resulting specification to grow exponentially. In this section we describe the Flattening and Recombination (FAR) algorithm that produces an equivalent specification that is shorter and more practical than the input specification. 


In this section we discuss the \FAR algorithm and soundness of the results produced by \FAR and develop a theorem about its soundness. We say that \FAR is \emph{sound} 
if the specification that results from running \FAR is equivalent to its argument specification. By \emph{equivalent} we mean that the set of programs satisfying the argument specification is the same as the set of programs satisfying the resulting specification. 

The outline of this section is as follows. First, in Section \ref{sec:specs-as-boolean-formulas}, we discuss the connection between JML specifications and first order Boolean formulas and describe our meaning of the specifications that \FAR operates on. As we shall discuss, the soundness of \FAR depends on the soundness of $\sim$, and in Section \ref{sec:soundness-of-tilde} we will discuss the soundness property of $\sim$ used in \FAR. Lastly, in Section \ref{sec:soundness-of-far} we discuss the soundness theorem of \FAR.


\subsection{Abstract Specifications}
\label{sec:specs-as-boolean-formulas}\label{sec:abstract-specifications}

In discussing the soundness of \FAR, it is useful to abstract the specifications \FAR operates on from particular specification languages. In this section we discuss the formal details of the kinds of specifications \FAR operates on and produces independent of a particular specification language.
The specifications themselves are to be thought of as method specifications.
The only interesting properties we assume about specfications are that one can extract cases (such as those produced by $SP$) from a specification
and that each such case has a set of preconditions (conceptually a conjunction) and a set of other clauses (also conjoined).
Thus each specification is modeled as a non-empty list of cases, separated by a special operator $\vee$.  
Within a case, each clause is modeled as an ``atomic formula,''
which can be thought of as an assertion whose structure is not further examined; $\FAR$ treats atomic formulas as variables.
Specifications allow preconditions to distribute over cases, but in specification normal form (SNF), which is the format of the output of $\SP$ and the input of $\FAR$, no such distribution of preconditions is allowed;
thus in SNF each case is a non-empty list of preconditions and other clauses, each separated by the operator $\wedge$. However, in specifications in general $\wedge$ can be used to distribute preconditions over other specifications.

The semantics of specifications is most easily understood for the simple case of SNF, where the intuition is that for a specification of the form 
$a \vee b \vee c$,
if the preconditions of each of the cases $a$, $b$, and $c$ are never true in the same pre-state, then an implementation that transforms a pre-state $s$ into a post-state $s'$ is correct if the pair of states $(s,s')$ satisfies the non-preconditions of the case whose precondition was true in the pre-state $s$. This semantics the same as JML's \lstinline!also! operator when the preconditions are disjoint, and the outputs of $SP$ and $\FAR$ always have disjoint preconditions.
A specification of the form $\CREATEDISTRIB{p}{S}$, is an abbreviation for distributing the precondition $p$ into each case of $S$, and thus simply adds the precondition $p$ to each specification case of $S$.

\begin{definition}[A Specification Language]
  \label{def:spec-language}
A \emph{specification language} is a language modeled by a set of expressions, $\EXP$, a set of type expressions, $\TYPEEXP$, that includes $\BOOLEAN$, a set of type environments, $\TYPEENV$, a typing judgment, $\vdash$, a set of states, $\STATE$, and, for each type environment $\Gamma \in \TYPEENV$ a meaning function for expressions, ${\cal E}_{\Gamma}$.
Type environments $\Gamma\in\TYPEENV$ are maps from names to $\TYPEEXP$.
Typing judgments of the form $\Gamma \vdash E : \tau$ relate a type environment ($\Gamma$), an expression ($E$), and a type expression ($\tau$).

Boolean-valued expressions are called \emph{atomic formula}:
\begin{displaymath}
\ATOMICFORMULA \DEF \{ E \mid E \in \EXP, \exists \Gamma \in \TYPEENV . \Gamma \vdash E : \BOOLEAN \}.
\end{displaymath}
Since some atomic formulas may relate a pre-state to a post-state,
the meaning function for expressions that type check in a type environment $\Gamma$, ${\cal E}_{\Gamma}$, takes two states as an argument.
For a given type environment $\Gamma$,
\emph{$\Gamma$-state}s $s$ and $s'$ are states that agree with the type environment $\Gamma$ in the sense that for each expression $E$, 
if $\Gamma \vdash E : \tau$, then $\ME{\Gamma}{E}(s,s')$ is an element of the meaning of the type $\tau$.

%A \emph{specification} follows the grammar shown in Figure~\ref{fig:spec-grammar}.
%\input{figures/spec-grammar}
\end{definition}

We use the notation $\CASES$ to extract the cases of a specification as a set.
\begin{displaymath}
\begin{array}{l}
\CASES : \SPECIFICATION \rightarrow \POWERSET{\CASE} \\
\CASES(S) \DEF \LETHEAD{c_1 \vee \ldots \vee c_n}{S} \{ c_1, \ldots, c_n \}      
\end{array}
\end{displaymath}

Sometimes it will be convenient to use operators $\PRE$ and $\REST$ to extract the precondition and other atomic formulas (e.g., the postcondition) from a case; they have types:
\begin{displaymath}
\begin{array}{l}
   \PRE : \CASE \rightarrow \POWERSET{\ATOMICFORMULA} \\
   \REST : \CASE \rightarrow \POWERSET{\ATOMICFORMULA}.
\end{array}
\end{displaymath}
These operations satisy, for all $P,Q \in \POWERSET{\ATOMICFORMULA}$, and $S\in\SPECIFICATION$,
\begin{align}
    \PRE(\CREATE{P}{Q}) & = P \\
    \REST(\CREATE{P}{Q}) & = Q \\
    \PRE(\CREATEDISTRIB{P}{S}) & = P \cup \left( \bigcup_{c\in\CASES{S}} \PRE(c)\right) \\
    \REST(\CREATEDISTRIB{P}{S}) & = \bigcup_{c\in\CASES{S}} \REST(c).
\end{align}

A restriction of the greneral form of specifications defines the output format of $\SP$ and thus the input format of $\FAR$. This format does not allow preconditions to be combined with specifications using $\wedge$.

%\begin{definition}[Specification Normal Form (SNF)]
%  \label{def:snf}
%A specification is in \emph{specification normal form (SNF)} if it follows the grammar in Figure~\ref{fig:snf-grammar}.
%\input{figures/snf-grammar}
%\end{definition}

\subsection{Connection with SP}

The foundation of the connection between a specification languages 
and the abstract specifications described in Section~\ref{sec:abstract-specifications}
and the formulas produced by $\SP$ is straightforward, because $\SP$ produces formulas in disjunctive normal form in which the formulas corresponding to preconditions are all disjoint.
%To illustrate this connection, the simple program, \texttt{cmp}, shown in Figure \ref{fig:cmp-normal}.
%
%\input{listings/cmp}
%
%The computation of $\SP(\texttt{cmp},\phi)$ produces the following formula:
%
%\begin{equation}\label{eqn:sp-computed}
%\begin{array}{l}
%  (a < b \land \phi \land \KW{result} = -1) \\
% ~ \lor \: ( (a > b \land \lnot(a < b) \land \phi \land \KW{result} = 1) \\
% ~ \lor \: (\lnot(a < b) \land \lnot (a > b) \land \phi \land \KW{result} = 0))
%\end{array}
%\end{equation}
%
%Formula~(\ref{eqn:sp-computed}) corresponds to the following abstract specification.
%
%\begin{equation}\label{eqn:sp-computed-spec}
%\begin{array}{l}
%  (\PREREST{a < b \land \phi}{\KW{result} = -1}) \\
% ~ \vee \: (\PREREST{a > b \land \lnot(a < b) \land \phi}{\KW{result} = 1}) \\
% ~ \vee \: (\PREREST{\lnot(a < b) \land \lnot (a > b) \land \phi}{\KW{result} = 0})
%\end{array}
%\end{equation}

Consider the contract in Listing \ref{fig:cmp-normal-spec}. In this contract, although the symbols are different, we can see terms that correspond to the terms found in the result of $\SP$ in formula (\ref{eqn:sp-computed}) and the corresponding abstract specification in formula (\ref{eqn:sp-computed-spec}). Specifically, note that the three parts of the JML specification that are separated by ``\KW{also}'' in Listing \ref{fig:cmp-normal-spec} correspond to the three cases (separated by $\vee$) of the abstract specification in formula (\ref{eqn:sp-computed-spec}). The translation to JML is very direct in this way.

For specification languages that do not have JML's specification cases it is still possible to use the output of FAR to make the specificaions shorter. This would be done by translating a formula like formula (\ref{eqn:sp-computed-spec}) into a single postcondition, using a translation function $\TR$ defined on specificaitons and cases as follows:

\begin{displaymath}
\begin{array}{l}
  \TR(c_1 \vee \ldots \vee c_n) = \TR(c_1) \land \ldots \land \TR(c_n) \\
  \TR(\PREREST{p}{q}) = (\OLD(p) \implies q) \\
  \TR(\PREDISTRIB{p}{S}) = (\OLD(p) \implies \TR(S))
\end{array}
\end{displaymath}

Note the use of $\land$ instead of $\vee$ in the produced postcondition to connect cases. If this were not done, then the postcondition would be trivially satisfied whenever one of the preconditions was false.
(Also for the distributed form of specification cases $\PREDISTRIB{p}{S}$,
note that $p \implies (p' \implies q)$ is equivalent to $p \land p' \implies q$, so the first precondition ($p$) distributes over the others as required.)
For example, formula (\ref{eqn:sp-computed-spec}) would turn into the following postcondition

\begin{equation}\label{eqn:sp-non-JML}
\begin{array}{l}
  (\OLD(a < b \land \phi) \implies (\KW{result} = -1)) \\
 ~ \land \: (\OLD(a > b \land \lnot(a < b) \land \phi) \implies (\KW{result} = 1)) \\
 ~ \land \: (\OLD(\lnot(a < b) \land \lnot (a > b) \land \phi) \implies (\KW{result} = 0))
\end{array}
\end{equation}

%\input{translation}

% \input{far-algorithm}

%\subsection{Description of FAR}

%The main pseudocode of FAR is given in Algorithm \ref{alg:far}. In this section we will discuss the main parts of the algorithm as they relate to Algorithms \ref{alg:far}, \ref{alg:mergescc}, \ref{alg:to-graph}, and \ref{alg:to-specification} and Figure \ref{fig:overview-pipeline}. The FAR algorithm has 4 main parts, described below. 
% 
%\textit{Input Specification}. The input to \FAR comes directly from the specification produced by the predicate transformer semantics. Since the specification is produced by $sp$, the specification will be in SNF. These clauses are placed in a data structure suitable for a graph-based analysis. For our implementation, we used the JPaul program analysis library \cite{jpaul}. This process happens on Line \ref{ln:far-inputspecification} of Algorithm \ref{alg:far}. 

%\textit{Flattening}. With the cases of the specification cases collected, the next step is to flatten the specification. This is done by taking each node of the input specification that is not a disjunction node and detaching it from the tree. This forms a disjoint forest of all the specifications cases. Once flattening is then complete, the algorithm computes weights using an equivalence relation on pairs of distinct vertices. Weighted edges are shown by the dashed arrows in Figure \ref{fig:overview-pipeline}. On Line \ref{ln:weights} of Algorithm \ref{alg:to-graph} this equivalence realtion is denoted by the symbol $\sim$ (see Section \ref{sec:soundness-of-tilde}). For simplicity, our prototype concludes that two clauses are equivalent if they are lexically identical. We show the soundness of this choice in Corollary \ref{lem:soundness-of-le}. In our experimental analysis (Section \ref{sec:technical-evaluation}) we find that this choice works out well. Note however that the relation used for FAR need not be lexical similarity; indeed, more interesting results can be achieved by considering other relations such as logical equivalence. 
%
%\textit{State Finding}. In the state finding phase (Lines \ref{ln:far-loop}-\ref{ln:far-loop3} of Algorithm \ref{alg:far}), the dashed arrows leaving each vertex are added together and converted to graph weights as can be seen in Figure \ref{fig:overview-pipeline}. For example, examining vertices $C_2$ and $C_3$ we see two edges going from $C_2$ to $C_3$. This means in the state finding phase we will place an edge with weight 2 between these two vertices. The algorithm continues in this fashion until it produces a weighted graph. Next, compute the connected components of this graph. In Figure \ref{fig:overview-pipeline}, this process produces Component 1 and Component 2. Then, for each connected component, select the pair of vertices with the largest weight (most similarity). In Figure \ref{fig:overview-pipeline} this produces the choice  $(C_6,C_7)$ for Component 1 and $(C_2,C3)$ for Component 2. 
 
%\textit{Recombining}. For each selected pair of vertices from the State Finding step we perform the following procedure (Lines \ref{ln:select-pair}-\ref{ln:replace-v2} of Algorithm \ref{alg:mergescc}): First, we create a conjunction node (a logical AND) and connect it to each vertex in the pair. We then modify each vertex in the pair in the following way. The right vertex becomes the conjunction of all of the clauses that were lexically equal in both vertices. The left vertex becomes the disjunction of the set of clauses that \textit{were not} lexically equal in both vertices. In Figure \ref{fig:overview-pipeline} this operation is denoted by the $*$ next to the vertex name. Next, we examine the connected component to which the pair belongs. If any vertex is adjacent to any of the elements of the pair, we remove that edge from the graph. This process is repeated for each connected component produced in the previous step. Lastly, we create a ``super node'', which will serve as the new root of the specification. This node should be a disjunction (logical OR) and be connected to the newly created conjunction nodes (the merged states in Figure \ref{fig:overview-pipeline}). In the example in Figure \ref{fig:overview-pipeline}, this leaves us with vertices $C_1$ and  $C_5$. This subgraph is then fed back into the FAR algorithm until there are no remaining vertices. Completely disjoint vertices (those with nothing in common with any of the other vertices) form a disjoint forest in the final iteration of the algorithm. Once this outcome is reached, each vertex in the forest is connected unmodified to the super node. This resulting tree is then converted back into a specification. 

%\subsection{Base Analysis Types}
%\label{sec:analysis-types}
%
%After an execution trace of a particular method is obtained, we next need to transform the trace and the underlying predicate AST into a practical contract. The portion of Strongarm that is responsible for this task is the various analyses in the contract transformation pipeline (see Figure \ref{fig:overview-pipeline}). These base analysis types include standard tasks such as translation from internal variable representations to externalized (source code level) representations, removal of tautologies, determination of purity, and inference of frame axioms. For space considerations we omit a detailed description of these standard techniques. 

\subsection{Soundness of $\sim$}
\label{sec:soundness-of-tilde}

The $\FAR$ algorithm uses an equivalence relation $\sim$ to compute
the intersection between two sets of preconditions. 
However, not just any equivalence relation on atomic formulas will do; the relation must preserve the meaning of atomic formulas.

\begin{definition}[Sound Equivalence Relation]
\label{def:tilde-r}
An equivalence relation $\sim$ on atomic formulas is \emph{sound} iff for all type environments $\Gamma$ and all atomic formulas $F$ and $G$ such that
$\Gamma \vdash F : \BOOLEAN$ and $\Gamma \vdash G : \BOOLEAN$:
\begin{displaymath}
  F \sim G \implies \forall \Gamma\textrm{-states } s, s' \: . \: 
     \ME{\Gamma}{F}(s,s') = \ME{\Gamma}{G}(s,s').
\end{displaymath}
\end{definition}

The $\FAR$ algorithm works correctly if $\sim$ is any sound equivalence relation on atomic formulas. However, in this paper and our implemention we use lexical equivalence (i.e., textual identity) as the relation,
hence we need the following corollary, whose proof is trivial.

\begin{corollary}[Soundness of Lexical Equivalence]
  \label{lem:soundness-of-le}
  Lexical equivalence of atomic formulas is a sound equivalence relation.
\end{corollary}

\subsection{Soundness of \FAR}
\label{sec:soundness-of-far}

In this section we show the soundness of \FAR. Since soundness for $\FAR$ is defined with respect to satisfaction by programs (method bodies), we first define satisfaction for programs. In essence the following definition says that a program $C$ satisfies a specification $S$ if for every pre-state $s$ that satisfies some case $c$'s precondition, the semantics of $C$ is such that the post-state $s'$ that $C$ produces (when run on $s$) satisfies $c$'s postcondition.

\begin{definition}[Satisfies a Specification] \label{def:models}
Let $\Gamma$ be a type environment. Let $S$ be a specification in which each atomic formula contained in $S$ type checks in $\Gamma$.
Let $C$ be a program whose semantics is captured by a state transformer $\chi$ that transforms $\Gamma$-states to $\Gamma$-states.
Then \emph{$C$ satisfies $S$}, written $C \MODELSWRT{\Gamma} S$,
if and only if for all $\Gamma$-states $s$ such that there is a case 
$c \in \CASES(S)$ such that for each atomic formula $p \in \PRE(c)$,
$\ME{\Gamma}{p}(s,s)$ is true,
and $\chi(s) = s'$, then for each atomic formula $q \in \REST(c)$,
$\ME{\Gamma}{q}(s,s')$ is true.
\end{definition}

% \begin{definition}[Specification Linkages]
% Let $q$ be an atomic formula contained in some case $\REST(c)$ of specification $S$. The preconditions that govern $q$ are the set of $\PRE(c)$. The tuple $\langle \PRE(c), \REST(c)\rangle$ form a \textit{specification linkage}, that is a requirement on $S$ such that $\REST(c)$ must be governed 
% \end{definition}

The following lemma relates to the invariant of the $\FAR$ algorithm that we use to prove its soudness.

\begin{lemma}[\ToSpecification on Flat Tree] \label{lem:flat-tree}
  Let $G$ be a graph $\langle V,E \rangle$ with root $G.root$ such that $\forall v \in V~ \langle G.root, v \rangle \in E$. Then $\ToSpecification(G, G.root)$ produces the disjunction of each $v \in V$.
  \end{lemma}
  \begin{proof}
    Let $G$ be a graph $\langle V,E \rangle$ with root $G.root$ such that $\forall v \in V~ \langle G.root, v \rangle \in E$. On Line \ref{ln:foreach-adjacent}, \ToSpecification iterates over each vertex in $G$. On Line \ref{ln:isaleaf}, we test if $v$ is a leaf. Since all $v$ are leaves, on return on Line \ref{ln:return-tospecification}, $B$ contains the set $V$. Since $\bigvee B$ produces the disjunction of every element of $B$, $\ToSpecification(G, G.root)$ produces the disjunction of each $v \in V$.
  \end{proof}
  
The following corollary also relates to the invariant in the $\FAR$ algorithm.
  
  \begin{corollary}[Two-Leaf Pairs Converted to Specifications]
    \label{col:logical-relation-of-any-two-v}
    Let $G$ be a graph $\langle V,E \rangle$ with root $G.root$. For any pair of leaf vertices $(l,r)$ adjacent to $G.root$, $\ToSpecification(G, G.root)$ contains a disjunction of $l$ and $r$ if and only if $\{l,r\} \subseteq V$.
  \end{corollary}
  

% \begin{lemma}[Specification Linkage] \label{lem:spec-link}
% Let $q$ be an atomic formula contained in some case $c$ of specification $S$. Then the set of preconditions that govern $q$ in $S$ is the same as the set of preconditions that govern $q$ in $\FAR(S)$. 
% \end{lemma}
% \begin{proof}
%   Go through algorithm...
% \end{proof}

The following definition of soundness for $\FAR$ is reasonable because if $\FAR$ does not change the meaning of a specification, then it is only simplifying it. Furthermore, since we pass specifications to $\FAR$ that are derived from $\SP$ and these capture the behavior of the code, if $\FAR$ does not change the meaning of these specifications, then they still capture the behavior of the code.

\begin{definition}[Soundness of \FAR]
\label{def:soundness-of-far}
Let $\sim$ be a sound equivalence relation on atomic formulas.
Then \emph{$\FAR$ is correct with respect to $\sim$} iff for all programs $C$ and for all specifications $S$:
    $$C \MODELSWRT{\Gamma} S \iff C \MODELSWRT{\Gamma} \FAR(S,\sim).$$
\end{definition}

\begin{theorem}[FAR is Sound]
  \label{theo:far-is-sound}
  If $\sim$ is a sound equivalence relation, then \FAR is correct with respect to $\sim$.
\end{theorem}
\begin{proof}
  Assume $\sim$ is a sound equivalence relation. Let $\Gamma$ be a type environment. Let $C$ be a command with semantics $\chi$ that takes $\Gamma\text{-states}$ to $\Gamma\text{-states}$. Let $S$ be a specification in SNF in which each atomic formula contained in $S$ typechecks in $\Gamma$. 

The proof uses a loop invariant maintained by \FAR. \FAR maintains the state of its execution according to the tuple $\langle S, V, Residual \rangle$, where $V$ is a list of unmerged vertices and $Residual$ is the residual graph formed from previous $MergeSCC$ calls. We refer to the state $\langle S, V, Residual \rangle$ as $\FAR_{State}$ and define the following invariant that operates on its elements: 

  \begin{displaymath}
    \begin{array}{l}
    \metaop{inv} : \SPECIFICATION \rightarrow \{Case\} \rightarrow Graph \rightarrow \BOOLEAN \\
    \metaop{inv}(S, V, G) \DEF \: \LETHEAD{G'}{\langle G.V \cup V, G.E \cup \{(G.root, v) ~|~ v \in V\} \rangle} \\ 
    ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \:  C \MODELSWRT{\Gamma} S \iff C \MODELSWRT{\Gamma} \FAR(\ToSpecification(G', G'.root),\sim)
      
    \end{array}
    \end{displaymath}
    
    The graph $G'$ formed in \metaop{inv} by $\langle G.V \cup V, G.E \cup \{(G.root, v) ~|~ v \in V\} \rangle$ encapsulates Lines \ref{ln:far-makeg-1} and \ref{ln:far-makeg-2} of \FAR which are responsible for taking the remaining elements of $V$ and adding them to the residual graph. As can be seen on Line \ref{ln:far-makeg-1} they are added to the root of $Residual$. Encapsulating the end of the \FAR procedure in this way demonstrates what a snapshot of the state of \FAR would be for any given iteration of the loop on Line \ref{ln:far-loop}. 
    
  \textit{Establishing.} The invariant \metaop{inv} is established after the execution on the statement on Line \ref{ln:inv-established} of Algorithm \ref{alg:far}. At this point $\FAR_{State} = \langle S, \CASES(S), \langle \emptyset, \emptyset \rangle\rangle$. In \metaop{inv}, since $G$ is empty, $G'$ is a graph with a root that is attached via an edge to each leaf in $V$. By Lemma \ref{lem:flat-tree}, we know that $\ToSpecification(G', G'.root)$ is the disjunction of all of the cases of $V$. While this may reorder the cases, the semantics of a speicification is unaffected by the order of the cases, therefore the invariant is established.  
  
  \textit{Maintaining.} Lines \ref{ln:far-loop1} and \ref{ln:far-loop2} have no effect on the values of $\FAR_{State}$ and therefore do not directly affect the value of \metaop{inv}. We are concerned with the effect of the computation on Line \ref{ln:far-loop3}. The result of Line \ref{ln:far-loop3} is impacted by the value of $V$, the value of which takes on several cases. 
  \begin{description}
    \item[Case 1] Consider $V = \emptyset$. In this case $\MergeSCC(V, W, Scc, Residual, \sim) = \langle V, Residual \rangle$. That is, $\langle V, Residual \rangle$ is not modified. This case is trivial since the connected component of an empty graph is empty as well. In this case $\langle V, Residual \rangle$ is not modified and hence $\FAR_{State}$ remains the same. 
    \item[Case 2] Consider $V \neq \emptyset$ and for every pair $(l,r) \in V \times V$  such that $l \neq r $ the formula $|\{ (x,y) \in \PRE(l) \times \PRE(r) ~|~ x \sim y\}| = 0$ is true. In this case, for each iteration of the loop of Algorithm \ref{alg:to-graph}, the condition on Line \ref{ln:to-graph-branch} is false. This case is equivalent to case 1, since there are no edges and therefore the graph is a disjoint forest. In this case, the connected components all contain one vertex. However, since the loop on Line \ref{ln:merge-loop} of Algorithm \ref{alg:mergescc} only executes in the event $|Component.V| > 1$, the pair $\langle V, Residual \rangle$ is not modified and hence $\FAR_{State}$ remains the same.

    %$$\forall (l,r) \in V \times V \text{ such that } l \neq r, |\{ (x,y) \in \PRE(l) \times \PRE(r) ~|~ x \sim y\}| = 0  $$

    \item[Case 3] Consider $V \neq \emptyset$ and there exists some pair $(l,r) \in V \times V \text{ such that } l \neq r $ where $|\{ (x,y) \in \PRE(l) \times \PRE(r) ~|~ x \sim y\}| > 0$. In this case, at least one component of $Scc$ will satisfy the requirement $|Component.V| > 1$ of the loop on line \ref{ln:merge-loop} of Algorithm \ref{alg:mergescc}. We consider the effect of a single component on the value of \metaop{inv}. Let the pair selected on Line \ref{ln:select-pair} be the pair $(L,R)$. Let $common$ be the set $\{ l ~|~ (l,r) \in \PRE(L) \times \PRE(R)$ where $l \sim r\}$ computed on Line \ref{ln:common} of Algorithm \ref{alg:mergescc}. On exit from Line \ref{ln:mergescc-remove-v} of Algorithm \ref{alg:mergescc} $\FAR_{State} = \langle S, V', Residual' \rangle$ where the following updates have been made:
    
    \begin{itemize}
      \item[] $V' = V \setminus (\{R\} \cup \{L\}) \implies \ToSpecification(Residual, Residual.root) $ does not contain $L \lor R$ (by Corollary \ref{col:logical-relation-of-any-two-v}), which causes \metaop{inv} to no longer hold. 
    \end{itemize}

However, the following computation causes \metaop{inv} to hold again: 

% \ShowLn   $R' \longleftarrow \PREREST{(\PRE(R) \setminus \{r ~|~ (l,r) \in \PRE(L) \times \PRE(R) \text{ where } l \Sim r\})}{\REST(R)} $\;

%    \ShowLn   $L' \longleftarrow \PREREST{pre(L) \setminus common}{rest(L)}$\;
 
\begin{itemize}
  \item[] $Residual'.E = Residual.E \cup (\{common\} \times \{L', R'\}) \cup \{(Residual.root, common)\}$
  \item[] $Residual'.V = Residual.V \cup \{L\} \cup \{R\}$
  \item[] $\mathbf{where} $
  \begin{itemize}
    \item[] $L' = \PREREST{(pre(L) \setminus common)}{rest(L)}$ 
    \item[] $R' = \PREREST{(\PRE(R) \setminus \{r ~|~ (l,r) \in \PRE(L) \times \PRE(R) \text{ where } l \sim r\})}{\REST(R)}$
  \end{itemize}
\end{itemize}

    On Line \ref{ln:mergescc-remove-v}, $L$ and $R$ are removed from $V$. Prior to removal, an evaluation of \metaop{inv} would produce a disjunction of $L$ and $R$ from Corollary \ref{col:logical-relation-of-any-two-v} in the final specification. They are replaced in $Residual$ by something that translates to an equivalent specification. That is, the formula  $(L \lor R)$ is replaced by $(common \land (L' \lor R'))$ on Lines \ref{ln:replace-v1} and  \ref{ln:replace-v2} when $Residual$ is updated. Since $\sim$ is a sound equivilance relation, $(L \lor R) \equiv (common \land (L' \lor R')) \implies \metaop{inv}(S,V,Residual)$ and therefore the invariant \metaop{inv} is maintained. 

  \end{description}

  \textit{Terminating.} In the case evaluation in the maintaining step, we showed how \metaop{inv} holds at each step of the loop in \FAR. Since Lines \ref{ln:far-makeg-1} and \ref{ln:far-makeg-2} are encapsulated by \metaop{inv}, we know that \metaop{inv} holds on exit from \FAR which gives us the desired result.
\end{proof}

% Local Variables:
% word-wrap: 1
% auto-fill-function: nil
% End:


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

% Outline
% -	Anything you thought of that should be in the paper but doesn’t fit. 
% -	Dynamic dispatch (why we don’t care!?) 
% -	Java’s extended for loop (why we don’t support it)
% -	Future work (extended for loops / integration with Boa / details about loops / framing / any assumptions we made / inferring our own loop invariants / handling exceptions) 
% o	LOOP PROBLEMS, BLACK BOX LIMITATIONS
% -	Java extended for loops



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> end-matter.tex <==
% \section{Future Work} \label{sec:future-work}

% \begin{enumerate}
%     \item Does the wrong kind of relation for $\sim_R$ cause FAR to be incorrect?
% \end{enumerate}

\section{Acknowledgments} \label{sec:acknowledgments}
The work of Anonymous Authors was supported in part \blackout{by NSF grants NNNNNNN and NNNNNN. The work of Anonymous Authors was also supported by NSF grants NNNNN and NNNNNN}.

This material is based upon work supported by the National Science Foundation under Grant No. \censor{NNNNNNN}. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.
  

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> eq-stuff <==


C1:     C2:
a       a'
b       b'
c       c'



a = a'
a = b' => b' = a'
b = b'
b = a 
b' = a 
c = c' 


[a] = [b]= {a,a',b'} 
[c] = {c,c'}

{l | (l, r) ∈ L × R such that l ∼ r}

Answer: {a,b,c}


Quotient Set:
(L \cup R)/~ = [a] \cup [b] \cup [c] \cup [a'] \cup [b'] \cup [c']

Representative Set: 

A set containing a rep. from each E.C. 

[a] = {a,a',b'} 
[b] = {a,a',b'}
[c] = {c,c'}

R_abc = {a,a',c}

==> execution-overview.tex <==
\section{Overview of Techniques for Inferring Specifications}
\label{sec:overview-of-execution-techniques}

(describe all the different types of execution models)

==> figures/all-analysis-types.tex <==

\renewcommand{\arraystretch}{2.6}
\begin{figure*}[]
\centering 

\begin{tabular}{llp{8cm}}
  \toprule
Analysis & Target AST & Description \\ 
\toprule
%  Remove Redundant Preconditions (RRP) & Specification & \parbox{8cm}{Removes preconditions in sub-cases implied by preconditions in parent clauses.} \\  
%Remove Impossible Specification Cases (RIS) & Specification & \parbox{8cm}{Takes into account both local and parent specification cases; removes cases that are not satisfiable.} \\ 

Perform Lexical Substitutions (LEX) & Predicate & \parbox{8cm}{Using the lexical substitution table, substitute known relations into the underlying equation.} \\ 

Remove Tautologies (RT) & Specification & \parbox{8cm}{Removes all non-falsifiable propositions from the specification.} \\ 

  Remove Contradictions (RC) & Specification & \parbox{8cm}{Removes unsatifiable propositions from the specification.} \\ 

  
Remove Useless Cases (RUC)  & Specification & \parbox{8cm}{If a specification case (after simplification) contains no clauses it is pruned from the specification.} \\ 

  
Remove Dead Assignments (RDA) & Specification & \parbox{8cm}{Removes all unused assignments (assignments made and not used before being reassigned).} \\ 

Perform Premap Substitutions (PRE) & Predicate & \parbox{8cm}{Using the premap substitution table, replaces variables in the underlying predicate AST with program variables.} \\  

Remove Non-Visible Variables (RNV) & Specification & \parbox{8cm}{Removes variables from the specification that are not visible to clients (e.g., local variables)} \\ 

Perform Backwards Propagation (PBP) & Specification & \parbox{8cm}{After substitution, the specification may contain additional equations which can be used to simplify the specification. This step performs these substitutions. } \\ 

  
Translate Internal Variables (TIV) & Specification & \parbox{8cm}{Replaces internal variable names from optimal passive form conversion to JML-specific variables.} \\ 

Remove Duplicate Assignments (RDA) & Specification & \parbox{8cm}{Removes same-value multiple assignments to variables from specification} \\ 

Remove Prestate Assignables (RPA) & Specification & \parbox{8cm}{Removes references to prestate (\texttt{\textbackslash old}) variables in \texttt{assignable} clauses.} \\ 

  
Remove Useless Postconditions (RUP)  & Specification & \parbox{8cm}{If a specification case (after simplification) contains no postconditions it is pruned from the specification.} \\ 

  
Infer Frame Axioms (IFA) & Specification & \parbox{8cm}{Determines regions of the heap that are modified by the method and adds appropriate clauses describing the modification.} \\ 


Determine Method Purity (DMP) & Specification & \parbox{8cm}{
Determines if the method being analyzed has no side effects; if so the purity modifier is added to the specification.} \\ 

Flattening and Reconstruction (FAR) & Predicate & \parbox{8cm}{Performs the final specification simplification using the FAR algorithm (see Section \ref{sec:far-algorithm}).} \\ 

  
\bottomrule
\end{tabular} 


\caption{Listing of all analysis types in Strongarm's contract transformation pipline.  Each analysis is listed in the order in which it is applied to the inferred specification.  }
\label{fig:all-analysis}
\end{figure*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


% pipeline_steps = [
%     "AFTER REMOVING DUPLICATE PRECONDITIONS (VIA SMT)",
%     "AFTER REMOVING IMPOSSIBLE SPECIFICATION CASES (VIA SMT)",
%     "AFTER PERFORMING LEXICAL SUBSTITUTIONS",
% #    "AFTER PERFORMING LEXICAL SUBSTITUTIONS II",
%     "AFTER REMOVING TAUTOLOGIES OF",
%     "AFTER REMOVING CONTRADICTIONS OF",
%     "AFTER PRUNING USELESS CLAUSES OF",
%     "AFTER REMOVING DEAD ASSIGNMENTS OF",
%     "AFTER PERFORMING OPTIMIZED PREMAP BLOCK SUBSTITUTIONS",
%     "AFTER PERFORMING ALL PREMAP BLOCK SUBSTITUTIONS",
%     "AFTER REMOVING LOCALS OF",
%     "AFTER REMOVING SPEC PUBLIC OF",
%     "AFTER DOING BACKWARDS PROPAGATION OF",
%     "AFTER SIMPLIFYING LABELS OF",
%     "AFTER REMOVING DUPLICATE ASSIGNMENTS OF",
%     "AFTER FIXING RESULTS",
%     "AFTER REMOVING CONTRADICTIONS II OF",    
%     "AFTER CLEANING PRESTATE ASSIGNABLES",
%     "AFTER REMOVING USELESS POSTCONDITIONS",
%     "AFTER PRUNING USELESS CLAUSES II OF",
%     "AFTER ADDING PURITY",
%     "AFTER REDUCTION ANALYSIS",
%    ]



==> figures/far-example.tex <==
\begin{figure}[h]
\begin{subfigure}{\textwidth}
  \centering

%\lstinputlisting[language=Java,basicstyle=\footnotesize\ttfamily]{listings/cmp-far-pre.java}
\LSTJMLFILESLICE{2-17}{listings/cmp-far-pre.java}
\caption{}
  \label{fig:far-pre}
\end{subfigure} \\

\begin{subfigure}{\textwidth}
  \centering
  %\lstinputlisting[language=Java,basicstyle=\footnotesize\ttfamily]{listings/cmp-far-post.java}

  \LSTJMLFILESLICE{2-16}{listings/cmp-far-post.java}

\caption{}   
  \label{fig:far-post}
\end{subfigure}

\caption{(a) A inferred specification before applying FAR. (b) A simplified specification produced by Strongarm after applying FAR. Note that in (b) the lexical structure has been changed and takes advantage of the fact that \lstinline!\!(a < b)! is true in multiple branches. }
\label{fig:far-example}



\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/figure1.tex <==
\begin{figure} 
\begin{subfigure}{.5\textwidth}
  \centering

\lstinputlisting[language=Java,basicstyle=\footnotesize\ttfamily]{listings/cmp-contract-pre.java}

\caption{}
  \label{fig:contract-pre-transformation}
\end{subfigure}% 
\begin{subfigure}{.5\textwidth}
  \centering
  \lstinputlisting[language=Java,basicstyle=\footnotesize\ttfamily]{listings/cmp-contract-post.java}
\caption{}   
  \label{fig:contract-post-transformation}
\end{subfigure}

\begin{subfigure}{\textwidth}
  \centering

\lstinputlisting[language=Java,basicstyle=\footnotesize\ttfamily]{listings/cmp-formula.java}

\caption{}
  \label{fig:contract-formula}
\end{subfigure}% 

\caption{(a) A inferred specification computed directly from symbolic execution alone. (b) A simplified specification produced by Strongarm. (c) Raw propositional formula computed from symbolic execution on an Optimal Passive Form program.}
\label{fig:contract-transformation}



\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/jml-to-prop.tex <==
\begin{figure*}[p] %[p]
    \begin{mdframed}
  
  \begin{equation*}
  \frac
      {\clz{JMLSpecCase\textsubscript{1}} \goesto \clz{JMLSpecCase\textsubscript{1}$^\star$}  \term \clz{JMLSpecCase\textsubscript{2}} \goesto \clz{JMLSpecCase\textsubscript{2}$^\star$}}
  %-----------------
      {\clz{JMLSpecCase\textsubscript{1}} ; \clz{JMLSpecCase\textsubscript{2}}  \goesto (\clz{JMLSpecCase\textsubscript{1}$^\star$}  \land \clz{JMLSpecCase\textsubscript{2}$^\star$})} ~ \textsc{TR-SC}
  \end{equation*}
  
  
  \begin{equation*}
  \frac
      {\clz{JMLSpecCase\textsubscript{1}} \goesto \clz{JMLSpecCase\textsubscript{1}$^\star$}  \term \clz{JMLSpecCase\textsubscript{2}} \goesto \clz{JMLSpecCase\textsubscript{2}$^\star$}}
  %-----------------
      {\{| \clz{JMLSpecCase\textsubscript{1}} \kwd{ also } \clz{JMLSpecCase\textsubscript{2}} |\} \goesto (\clz{JMLSpecCase\textsubscript{1}$^\star$}  \lor \clz{JMLSpecCase\textsubscript{2}$^\star$})} ~ \textsc{TR-A}
  \end{equation*}
  
  
  
  \begin{equation*}
  \textsc{TR-Req1} ~ \frac
      {}
  %-----------------
      {V \ts \sigma\thicksim(\kwd{requires } \alpha) \goesto x:V } ~ \text{if } \sigma \in \mathbf{dom}(V) \land V( \sigma ) = x
  \end{equation*}
  
  
  \begin{equation*}
  \textsc{TR-Ens1} ~ \frac
      {}
  %-----------------
      {V \ts \sigma\thicksim(\kwd{ensures } \alpha) \goesto x:V } ~ \text{if } \sigma \in \mathbf{dom}(V) \land V( \sigma ) = x
  \end{equation*}
  
  \begin{equation*}
  \textsc{TR-Assn1} ~ \frac
      {}
  %-----------------
      {V \ts \sigma\thicksim(\kwd{assignable } \alpha) \goesto x:V } ~ \text{if } \sigma \in \mathbf{dom}(V) \land V( \sigma ) = x
  \end{equation*}
  
  
  \begin{equation*}
  \textsc{TR-Req2} ~ \frac
      {\text{if }  \sigma \not\in \mathbf{dom}(V) \land 
      y \not\in \mathbf{range}(V) \land V' = V[\sigma \mapsto y]}
  %-----------------
      {V \ts \sigma\thicksim(\kwd{requires } \alpha) \goesto y:V' } 
  \end{equation*}
  
  
  
  
  \begin{equation*}
  \textsc{TR-Ens2} ~ \frac
      {\text{if }  \sigma \not\in \mathbf{dom}(V) \land 
      y \not\in \mathbf{range}(V) \land V' = V[\sigma \mapsto y]}
  %-----------------
      {V \ts \sigma\thicksim(\kwd{ensures } \alpha) \goesto y:V' }  
  \end{equation*}
  
  
  
  
  
  \begin{equation*}
  \textsc{TR-Assn2} ~ \frac
      {\text{if }  \sigma \not\in \mathbf{dom}(V) \land 
      y \not\in \mathbf{range}(V) \land V' = V[\sigma \mapsto y]}
  %-----------------
      {V \ts \sigma\thicksim(\kwd{assignable } \alpha) \goesto y:V' } 
  \end{equation*}
  
    \end{mdframed}
    
  
  
  \caption{Translation rules for translating JML specifications to the propositional form. We use the notation $\sigma \thicksim \mathit{expr}$ to mean that the variable $\sigma$ may be substituted for $e$ in the side condition of the rule.}
  \label{fig:jml-to-prop}
  \end{figure*}
  
  % /*@
  %    public normal_behavior
  %      requires true; 
  %      {|
  %        requires (a < b); 
  %        ensures \result == -1; 
  %      also
  %      {|
  %        requires !(a < b); 
  %        requires (a > b); 
  %        ensures \result == 1; 
  %      also
  %        requires !(a < b); 
  %        requires !(a > b); 
  %        ensures \result == 0; 
  %    |}
  %   |}
  % */
  

==> figures/prop-to-jml.tex <==
\begin{figure*}[ht] %[p]
    \begin{mdframed}
  
  \begin{equation*}
  \frac
      {\clz{CExp\textsubscript{1}} \goesto \clz{JMLSpecCase\textsubscript{1}}  \term \clz{CExp\textsubscript{2}} \goesto \clz{JMLSpecCase\textsubscript{2}}}
  %-----------------
      {(\clz{CExp\textsubscript{1}} \land \clz{CExp\textsubscript{2})}  \goesto \clz{JMLSpecCase\textsubscript{1}}  ; \clz{JMLSpecCase\textsubscript{2}}} ~ \textsc{TR-P-SpecCase}
  \end{equation*}
  
  
  \begin{equation*}
  \frac
      {\clz{CExp\textsubscript{1}} \goesto \clz{JMLSpecCase\textsubscript{1}}  \term \clz{CExp\textsubscript{2}} \goesto \clz{JMLSpecCase\textsubscript{2}}}
  %-----------------
      { (\clz{CExp\textsubscript{1}}  \lor \clz{CExp\textsubscript{2}}) \goesto \{| \clz{JMLSpecCase\textsubscript{1}} \kwd{ also } \clz{JMLSpecCase\textsubscript{2}} |\} } ~ \textsc{TR-P-Also}
  \end{equation*}
  
  
  
  \begin{equation*}
  \textsc{TR-P-Stmt} ~ \frac
      {}
  %-----------------
      {V \ts x \goesto V(x) } ~ \text{if } x \in \mathbf{dom}(V)
  \end{equation*}
  
  
    \end{mdframed}
    
  
  
  \caption{Translation rules for translating the propositional form back to JML specifications.}
  \label{fig:prop-to-jml}
  \end{figure*}
  
  % /*@
  %    public normal_behavior
  %      requires true; 
  %      {|
  %        requires (a < b); 
  %        ensures \result == -1; 
  %      also
  %      {|
  %        requires !(a < b); 
  %        requires (a > b); 
  %        ensures \result == 1; 
  %      also
  %        requires !(a < b); 
  %        requires !(a > b); 
  %        ensures \result == 0; 
  %    |}
  %   |}
  % */
  

==> figures/spec-grammar.tex <==
\setlength{\grammarparsep}{2pt} % increase separation between rules
\setlength{\grammarindent}{6em} % increase separation between LHS/RHS 


\begin{figure}[ht]

  \begin{mdframed}
    \begin{grammar}

    <Specfication> ::= \clz{Case} \alt \clz{Case} $\vee$ \clz{Specification}
    \alt (\KW{pre} \clz{AtomicFormulas}) $\wedge$ \clz{Specification}

    <Case> ::= \KW{pre} \clz{AtomicFormulas}; \KW{rest} \clz{AtomicFormulas}

    <AtomicFormulas> ::= \clz{AtomicFormula} \alt \clz{AtomicFormula} $\wedge$ \clz{AtomicFormulas}
    \end{grammar}
  \end{mdframed}
  
  \caption{The abstract syntax of specifications.}
  \label{fig:spec-grammar}
\end{figure}



==> figures/substitution-scheme.tex <==


\begin{figure}[ht] 

  
  \centering

\includegraphics[scale=.9]{figures/substitution-scheme}

\caption{Strongarm performs manipulations to both the AST of the original boolean formula derived from applying the predicate transformer semantics as well as the AST that represents the final specification. Picking which tree to manipulate is a tradeoff; the grammar of the predicate AST is easier to manipulate whereas the AST of the specification contains more details specific to the target specification language. To ensure both ASTs have access to the underlying originating block information, the predicate AST uses a simple attribute grammar to maintain the block mapping information.}
\label{fig:substitution-scheme}



\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/syntax-jml.tex <==
\setlength{\grammarparsep}{2pt} % increase separation between rules
\setlength{\grammarindent}{6em} % increase separation between LHS/RHS 
 
\begin{figure}

  \begin{mdframed}
    \begin{grammar}

      <CExp> ::= \clz{CExp} $\land$ \clz{CExp}
      \alt \clz{CExp} $\lor$ \clz{CExp}
      \alt \clz{JMLSpecCase}

      <JMLSpecCase> ::= \clz{JMLSpecCase\textsubscript{1}} \clz{JMLSpecCase\textsubscript{2}}
      \alt \{| \clz{JMLSpecCase\textsubscript{1}} \kwd{also} \clz{JMLSpecCase\textsubscript{2}} |\}
      \alt \clz{JMLClauseExpr}

      <JMLClauseExpr> ::= \kwd{requires} $\alpha$
      \alt \kwd{ensures} $\alpha$
      \alt \kwd{assignable} $\psi$


    \end{grammar}
  \end{mdframed}
  
  \caption{Abstract syntax for a minimal subset of JML. Elements of the syntatic class CExp are used as connectives between JMLSpecCases. The JMLSpecCase and JMLClauseExpr syntatic classes serve as a minimal grammar for JML.}
  \label{fig:syntax-jml}
\end{figure}


==> keywords.tex <==


\subjclass{D.1.5 Object-oriented Programming, D.2.4 Software/Program Verification}% mandatory: Please choose ACM 1998 classifications from http://www.acm.org/about/class/ccs98-html . E.g., cite as "F.1.1 Models of Computation". 
\keywords{specification inference, JML, strongarm, predicate transformers, deductive verification}% mandatory: Please provide 1-5 keywords
% Author macros::end %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Editor-only macros:: begin (do not touch as author)%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\EventEditors{John Q. Open and Joan R. Acces}
\EventNoEds{2}
\EventLongTitle{European Conference on Object-Oriented Programming (ECOOP 2018)}
\EventShortTitle{ECOOP 2018}
\EventAcronym{ECOOP}
\EventYear{2018}
\EventDate{December 24--27, 2016}
\EventLocation{Little Whinging, United Kingdom}
\EventLogo{}
\SeriesVolume{42}
\ArticleNo{23}
% Editor-only macros::end %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> listings/cmp.tex <==
\begin{figure*}[ht] 
  \begin{subfigure}[t]{.49\linewidth}
    \LSTJMLFILESLICE{1-16}{listings/cmp-normal.java}      
    \caption{The code for a simple comparison function.} 
    \label{fig:cmp-normal}
  \end{subfigure} 
  \hspace*{\fill}
  \begin{subfigure}[t]{.49\linewidth}
    \LSTJMLFILESLICE{3-18}{listings/cmp-contract.java}
    \caption{The specification computed by $sp$ for \texttt{cmp}.}
    \label{fig:cmp-normal-spec} 
  \end{subfigure}

\caption{(a) The Java code for a simple comparison function. Using the
standard definition of strongest postconditions, one obtains the
postcondition shown in (b) for \texttt{cmp}.}
\end{figure*}



==> obey.tex <==
%{obey}

% \myobeycr is same as \obeycr, but doesn't do a \@gobblecr.
{\catcode`\^^M=13 \gdef\myobeycr{\catcode`\^^M=13 \def^^M{\\}}%
\gdef\restorecr{\catcode`\^^M=5 }}

% \obeytabs
{\catcode`\^^I=13 \gdef\obeytabs{\catcode`\^^I=13 \def^^I{\hbox{\hskip 4em}}}}

% \obeyspaces
{\obeyspaces\gdef {\hbox{\hskip0.5em}}}

% environment for displayed text, indented, obeys cr, tab, spaces
\newenvironment{obeyDisplay}{%
\samepage%
\begin{list}{}{}\item\obeyspaces\obeytabs\obeycr}{%
\end{list}}



==> specs-as-graphs.tex <==

    
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% word-wrap: 1
%%% auto-fill-function: nil
%%% End:


==> translation.tex <==
%In Section \ref{sec:jml-to-prop} we provide the semantics for translating to and from the specification form described in this section.

\input{figures/syntax-jml}

%\input{figures/jml-to-prop}
%\input{figures/prop-to-jml}


\subsubsection{Translation of $SP$ and JML Specifications}
\label{sec:jml-to-prop}


In this section we discuss the translation semantics for translating JML specifications to and from the propositional form. We give a listing of our translation semantics in Figures \ref{fig:jml-to-prop} and \ref{fig:prop-to-jml}.

As mentioned in Section \ref{sec:specs-as-boolean-formulas}, one of the important aspects of our approach to performing JML specification translation is that we treat the individual statements of the specification as opaque, i.e., we do not consider the meaning of the expression contained within a \textbf{\texttt{requires}} statement. Rather, we treat them as opaque propositions to be translated. This impacts our translation semantics and necessitates the creation of a variable store which will keep track of these associations. We define a variable store, $V$ as follows: 
\begin{equation}
V = \{[x \mapsto v]\}
\label{eqn:v-defn}
\end{equation}

For each of the members of the semantic class \clz{JMLClauseExpr} we define two forms of the translation function. The first form, e.g., \textsc{TR-Req-1}, converts the given \clz{JMLClauseExpr} to an opaque variable and requires that the expression has been previously converted. The opaque variable that is used is reused from the previous association of the expression within the variable store. The second form, e.g., \textsc{TR-Req-2}, does not require that the given \clz{JMLClauseExpr} has been previously defined. Instead it associates a fresh variable name with the given expression in the variable store. 

Additionally, in our translation semantics we make use of a special notation: 

\begin{equation}
  \sigma \thicksim \mathit{expr}
\end{equation}

The meaning of this notation is that $\sigma$ acts as a synonym for $\mathit{expr}$ and it is used in the translation rules that require the use of the variable store $V$.

